ByteComp: Revisiting Gradient Compression in Distributed Training

Gradient compression (GC) is a promising approach to addressing the communication bottleneck in distributed deep learning (DDL). However, it is challenging to find the optimal compression strategy for applying GC to DDL because of the intricate interactions among tensors. To fully unleash the benefits of GC, two questions must be addressed: 1) How to express all compression strategies and the corresponding interactions among tensors of any DDL training job? 2) How to quickly select a near-optimal compression strategy? In this paper, we propose ByteComp to answer these questions. It first designs a decision tree abstraction to express all the compression strategies and develops empirical models to timeline tensor computation, communication, and compression to enable ByteComp to derive the intricate interactions among tensors. It then designs a compression decision algorithm that analyzes tensor interactions to eliminate and prioritize strategies and optimally offloads compression to CPUs. Experimental evaluations show that ByteComp can improve the training throughput over the start-of-the-art compression-enabled system by up to 77% for representative DDL training jobs. Moreover, the computational time needed to select the compression strategy is measured in milliseconds, and the selected strategy is only a few percent from optimal.

==> implementaion.tex <==
\section{Implementation}

% \begin{figure}[t!]
% \begin{center}
% \centerline{\includegraphics[width=0.65\columnwidth]{figures/byteComp.pdf}}
% \caption{The \name~architecture. The blue part is added by \name.}% GC is short for gradient compression and CCL is short for collective communication library.}
% \label{fig:arch}
% \end{center}
% \end{figure}

{\name} has three components: the scheduler, gradient compression libraries, and collective communication libraries (CCL). 
It has 5.1K and 4.1K lines of code in C++ and Python.
% as shown in Figure~\ref{fig:arch}.

\noindent \textbf{\name~scheduler.}
Given a DDL training job and a GC algorithm, {\name} determines the compression option of each tensor based on Algorithms~\ref{algo:gpu} and \ref{algo:cpu}.
It adds hooks to DNN training frameworks, such as PyTorch~\cite{pytorch} and TensorFlow~\cite{tensorflow}. 
When a tensor is ready for communication, {\name} chooses the corresponding compression library and CCL for GC at runtime.

% \subsection{The Compression Libraries}
\noindent \textbf{The compression libraries.}
{\name} implements two compression libraries to support GC with GPUs and CPUs, respectively.
% \noindent \textbf{GPU GC library.}
% The GPU GC library consists of several popular compression algorithms~\cite{dgc, efsignsgd, 1bit, sparse2018gradient, stich2018sparsified, signum, wen2017terngrad, QSGD} and two error-feedback mechanisms~\cite{efsignsgd, dgc}. 
% GPU compression library is wrapped with Python APIs to launch GPU kernels for both the compression and decompression operations.
Because each GPU can receive multiple compressed tensors after communication if they are not allreducible, {\name} fuses the decompression operations for better performance.
The CPU GC library is accelerated with two types of parallelism.
Firstly, it launches multiple jobs for compression and decompression operations to achieve inter-task parallelism.
These jobs run simultaneously on different CPU threads.
Secondly, SIMD instructions and OpenMP are enabled to achieve intra-task parallelism.


% \subsection{The Communication Libraries}
\noindent \textbf{The communication libraries.}
{\name} has two CCL for DDL: CCL for tensors allreducible and not allreducible.
There are four communication patterns and {\name} breaks the communication into multiple phases.
In each phase, {\name} chooses from the two CCL libraries for communication according to the data format of compressed tensors.
Collective operations for intra-machine communication is implemented with NCCL and for inter-machine communication is implemented with both NCCL and \texttt{push\_pull()} in BytePS~\cite{byteps}.
Multiple CUDA streams are used to overlap the computation, communication, and compression. 
\vspace{-0.1in}
